Programming droplet motion using metamaterials

Motion control of droplets has generated much attention for its applications to microfluidics, where precise control of small fluid volumes is an imperative requirement. Mechanical vibrations have been shown to be effective at inducing controllable depinning, and activation of different drop motion regimes. However, existing vibration-based strategies involve establishing homogeneous rigid-body dynamics on the substrate, and therefore lack any form of spatial heterogeneity and tuning. Addressing this limitation, metamaterials provide an ideal platform to achieve spectrally and spatially selective drop motion control, which leverages their ability to attenuate vibrations in selected frequency bands and in selected regions of a substrate. In this work, we illustrate the potential of metamaterials-based drop control by experimentally demonstrating a variety of drop motion capabilities on the surface of metaplates endowed with locally resonant stubs. The experiments leverage the design versatility of a LEGO component-enabled reconfigurable design platform and laser vibrometry measurements with high spatial resolution.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}
